Exponential Stochastic Inequality

We develop the concept of exponential stochastic inequality (ESI), a novel notation that simultaneously captures high-probability and in-expectation statements. It is especially well suited to succinctly state, prove, and reason about excess-risk and generalization bounds in statistical learning, specifically, but not restricted to, the PAC-Bayesian type. We show that the ESI satisfies transitivity and other properties which allow us to use it like standard, nonstochastic inequalities. We substantially extend the original definition from Koolen et al. (2016) and show that general ESIs satisfy a host of useful additional properties, including a novel Markov-like inequality. We show how ESIs relate to, and clarify, PAC-Bayesian bounds, subcentered subgamma random variables and *fast-rate conditions* such as the central and Bernstein conditions. We also show how the ideas can be extended to random scaling factors (learning rates).

==> old.tex <==
\begin{definition}
We say that a family of random variables $\{U_f : f \in \cF \}$ satisfies the {\em strong Bernstein condition\/} if there is a $B > 0$ such that for all $f \in \cF$, $\E[U^2_f] \leq B \E[U_f]$ 
\end{definition}

We say that it is a {\em regular\/} (super)strong ESI family if it is (super)strong and additionally 
\begin{equation}
    \label{eq:strongmetaesiregularity}
\text{There is $\delta > 0$ such that:\ } \sup_{f \in \cF} \E[|X_f|^{2+\delta}] < \infty 
\end{equation}


If furthermore the small-ball type condition (\ref{eq:smallball}) holds for the family $\{X_f: f \in \cF \}$ or for the family $\{ X_f^+: f \in \cF \}$, then there exists $C' > 0$ such that for  all $0 < \eta < \eta^\circ$, all $f \in \cF$,
\begin{equation}\label{eq:strongesiregularity}
\E[X_f^2 \exp(\eta X_f)] {\leq} C'   \cdot \E[X_f^2].
\end{equation}

\begin{lemma}
    \label{lem:smallball}
    TODO CHECK WITNESS OF BADNESS
    Let $Z$ be a nonnegative random variable with bounded second moment $\overline{z^2} := {\bf E}[Z^2] < \infty$. Then for all $\delta > 0$, all $0 < c < 1$, if we pick $K= c^{-(1+\delta)/\delta} \cdot \bar{z^2}$, then it holds that  
    \begin{equation}\label{eq:firstball}
        {\bf E} [\ind{Z \geq K} Z] \leq c \cdot  ({\bf E}[ \ind{Z \geq K} Z])^{1-\delta}.
    \end{equation}
and also, with $C= 1/(1-c)$,  
 \begin{equation}\label{eq:secondball}
        {\bf E} [Z]  \leq C {\bf E}[\ind{Z < K} Z].
    \end{equation}
\end{lemma}

\begin{proof}
For all $0 < \gamma < 1$, $K > 0$, all $p > 0, q > 0$ with $1/p + 1/q=1$,  we have, by H\"older's inequality:
\begin{align*}
&    {\bf E}[\ind{Z \geq K} Z] =
{\bf E}[\ind{Z \geq K} Z^{1-2 \gamma} Z^{2\gamma}] 
\\
& \leq \left( {\bf E}[(\ind{Z \geq K} Z^{1-2 \gamma})^p]\right)^{1/p}
\cdot \left( {\bf E}[Z^{q 2\gamma}] \right)^{1/q} 
\end{align*}
Taking  $\delta= \gamma/(1-\gamma)$ so that 
$1-\delta = (1-2 \gamma)/(1-\gamma)$
and  $p= (1-\gamma)/(1- 2\gamma)$ and hence $q = (1-\gamma)/\gamma$, 
and reasoning analogously to the proof of Markov's inequality and finally using Jensen's inequality, 
we see that we can further bound:
\begin{align*}
&    {\bf E}[\ind{Z \geq K} Z] \leq 
 \left( {\bf E}[(\ind{Z \geq K} Z^{1 -\gamma})]\right)^{(1-2 \gamma)/(1-\gamma)}
\cdot \left( {\bf E}[Z^{2(1-\gamma)}] \right)^{\gamma/(1-\gamma)} \leq 
\\ & 
 \left( {\bf E}[(\ind{Z \geq K} 
 \frac{Z^{\gamma}}{K^{\gamma}} \cdot 
 Z^{1 -\gamma})]\right)^{(1-2 \gamma)/(1-\gamma)}
\cdot \left( {\bf E}[Z^{2(1-\gamma)}] \right)^{\gamma/(1-\gamma)} 
\leq  K^{- \gamma} \left( {\bf E}[\ind{Z \geq K} Z]
 \right)^{1-\delta} \cdot  \left({\bf E}[Z^2] \right)^{\gamma} 
 \\ &  = c \cdot \left( {\bf E}[\ind{Z \geq K} Z]
 \right)^{1-\delta}, 
\end{align*}
if we set $K= c^{-1/\gamma} \cdot \overline{z^2} =c^{-(1+\delta)/\delta} \cdot \overline{z^2}$. This proves (\ref{eq:firstball}). For (\ref{eq:secondball}), note that (\ref{eq:firstball}) can be rewritten as 
$$ 
\E[\ind{Z \geq K} Z] \leq c \E[\ind{Z \geq K} Z] +
c \E[\ind{Z < K} Z] 
$$
Rearranging gives that 
$
(1- c) \E[\ind{Z\geq K} Z] \leq 
c \E[\ind{Z < K } Z] 
$. Adding $(1-c)  \E[\ind{Z <  K} Z]$ to both sides
gives 
$$ 
(1-c) \E[Z] \leq  \E[\ind{Z < K} Z] 
$$
and the result follows. 
\end{proof}
As an aside, we note that (\ref{eq:wob}) is quite similar to the {\em witness-of-badness condition\/} of \cite{grunwald_fast_2016}; it would be interesting to check if the conditions can be unified. 

